A Video-Based Method for Objectively Rating Ataxia

For many movement disorders, such as Parkinson's disease and ataxia, disease progression is visually assessed by a clinician using a numerical disease rating scale. These tests are subjective, time-consuming, and must be administered by a professional. This can be problematic where specialists are not available, or when a patient is not consistently evaluated by the same clinician. We present an automated method for quantifying the severity of motion impairment in patients with ataxia, using only video recordings. We consider videos of the finger-to-nose test, a common movement task used as part of the assessment of ataxia progression during the course of routine clinical checkups. Our method uses neural network-based pose estimation and optical flow techniques to track the motion of the patient's hand in a video recording. We extract features that describe qualities of the motion such as speed and variation in performance. Using labels provided by an expert clinician, we train a supervised learning model that predicts severity according to the Brief Ataxia Rating Scale (BARS). The performance of our system is comparable to that of a group of ataxia specialists in terms of mean error and correlation, and our system's predictions were consistently within the range of inter-rater variability. This work demonstrates the feasibility of using computer vision and machine learning to produce consistent and clinically useful measures of motor impairment.

==> sections/0_abstract.tex <==
For many movement disorders, such as Parkinson's disease and ataxia, disease
progression is visually assessed
by a clinician using a numerical disease rating scale.
These tests are subjective, time-consuming, and must be administered
by a professional. This can be problematic where specialists are not available, or when a patient is not consistently evaluated by the same clinician. We present an automated method for
quantifying the severity of motion impairment in patients with ataxia, using only
video recordings. We consider videos of the finger-to-nose test, a common
movement task used as part of the assessment of ataxia progression during the course of routine
clinical checkups.

Our method uses neural network-based pose estimation and optical flow techniques to track the
motion of the patient's hand in a video recording. We extract features that
describe qualities of the motion such as speed and variation in performance.
Using labels provided by an expert clinician, we train a supervised
learning model that predicts severity
according to the Brief Ataxia Rating Scale (BARS). 
The performance of our system is comparable to 
that of a group of ataxia specialists in terms of mean
error and correlation, and our system's predictions were consistently within the range of
inter-rater variability. 
This work demonstrates the feasibility of using computer vision and machine learning to produce consistent and clinically useful measures
of motor impairment.



==> sections/1_intro.tex <==
\section{Introduction}
Tens of millions of people are affected by movement disorders in the US and Europe
alone, and this
number is projected to double in the next few decades
\citep{bach2011projected}.
Quantifying the severity of motor incapacity is useful
in monitoring the progression of these diseases and measuring the
effectiveness of treatments. Estimates of motor incapacity are most commonly 
made using questionnares, or visual assessments combined with numerical rating scales
\citep{goetz2008movement,schmahmann2009development,schmitz2006scale}. While
these rating scales have been shown to be useful, the
tests must be administered by an experienced clinician and are subjective. An automated,
objective measurement of severity would provide more consistent evaluations, particularly where specialists are not available.

We use computer vision and machine learning techniques to create an automated, video-based method for quantifying the severity of
motor impairment in patients with ataxia. The term \textit{ataxia} describes a heterogenous group of neurodegenerative
diseases characterized by gait incoordination, involuntary
extremity and eye movements, and difficulty in articulating speech \citep{klockgether2010sporadic}. The severity of ataxia is
typically assessed using motor function tests such as the finger-to-nose maneuver,
in which a patient alternates between touching his/her nose and the
clinician's outstretched finger. A neurologist observes  the patient's action and rates the
disease severity on a numeric scale such as the Brief Ataxia Rating Scale
(BARS) \citep{schmahmann2009development}. These rating scales often consider aspects of the
patient's movement such as speed, smoothness, and accuracy. This evaluation typically happens during regularly scheduled clinical visits, and is time-consuming for the neurologist. Furthermore, the rating assigned to the patient often varies from rater to rater \citep{weyer2007reliability}.
An automated, consistent method for rating ataxia can greatly alleviate
these problems.

Our work focuses on
video recordings of a patient performing the finger-to-nose test; such videos might be collected during a routine clinical visit, or even in the patient's home. This poses two main challenges. First, our system must be robust to the issues raised by video quality. Clinical videos are likely to be captured with a handheld camera, and may contain camera movements such as panning and zooming. Different clinical settings could produce variations in viewing angle and lighting conditions. A more fundamental challenge in this task is that the amount of data is limited, as is common in many clinical problems. Consequently, we must rely on machine learning techniques that work with limited amounts of training data. 

Our contribution is a video-based system that automatically produces ratings of
motor incapacity for ataxic patients. Our system is: (1) observer-independent, (2) as accurate as human raters, who are the current gold standard for such a task, and
(3) robust to the quality of videos taken in clinical settings. Our system combines optical flow and neural network-based pose estimation techniques to robustly track the
location of the patient's wrist and head in each video. To facilitate training on our small dataset, we designed features based on the motion characteristics described in the BARS rating criteria. We extract these features
from the wrist location signal, and use them in a learning algorithm to build a model
that predicts the BARS severity rating of the patient's action.
We selected a representative subset of our data to be rated by a group of
experienced ataxia specialists, and found that our system performed comparably
to the specialists. 

%$78\%$ of the time, our system's predictions fell within the range of inter-rater
%variability, and it was within one rating step for all
%but one video.

This work demonstrates the feasibility of an automated
method for assessing the severity of motor impairment in ataxic patients. Such a
system could be useful in clinical or even home settings by allowing more
frequent and more consistent assessments of the disease, or in clinical trials where consistency is required. The system would be
particularly useful in areas where a neurologist specializing in ataxia is
not available, which is the case in most parts of the country and the rest of the world. 



==> sections/2_relatedworks.tex <==
\section{Related Work}
\subsection{Ataxia Rating Scales}
Ataxias are a group of neurodegenerative
movement disorders characterized by incoordination of the extremities,
eyes and gait \citep{schmahmann2004disorders,klockgether2010sporadic}. Since their
introduction, quantitative rating scales have been the norm for ataxia
severity assessment. Examples of these scales include the International
Cooperative Ataxia Rating scale (ICARS), and the Scale for the Assessment and
Rating of Ataxia (SARA) \citep{trouillas1997international,schmitz2006scale}.
These scales require an expert clinician to visually assess the qualities of the
patient's movements and determine a numerical rating, a time-consuming process. In 2009, the Brief Ataxia Rating Scale (BARS) was
developed as a quantitative scale that is sufficiently fast and accurate for clinical
purposes. Nonetheless, as the designer of the BARS says, an observer-independent,
fine-grained method for assessing ataxia is still ``sorely
needed'' \citep{schmahmann2009development}. This work is the
first step towards such a method.

\subsection{Human Motion Analysis}

The use of camera systems to measure and detect pathological movement is
well-studied for many diseases \citep{sutherland2002evolution,galna2014accuracy}. These systems
typically utilize multiple camera setups along with passive or active markers
and other sensing methods such as electromyography to track the motion of the
subject \citep{muro2014gait,kugler2013automatic,lizama2016use}. Such camera setups are expensive and complicated, must be operated by expert technicians,
and often require expert interpretation. These requirements prevent the
use of these systems in clinical settings.
In this work, we
focus on monocular consumer-quality videos, since their ubiquity could enable widespread applications of our technique in both clinical and home
settings.

To the best of our knowledge, this is the first work that uses monocular video
recordings to automatically assess the severity of a neurological movement
disorder. Most existing approaches rely on more specialized hardware, and solve different problems:
they measure movements but do not produce a rating of disease severity
\citep{galna2014accuracy}, or they focus on differentiating healthy and impaired
patients \citep{fazio2013gait,weiss2011toward}. One exception is the work by
\citeauthor{giuffrida2009clinically}, which produces a Unified Parkinson's
Disease Rating Scale rating from inertial sensor data
\citep{giuffrida2009clinically,goetz2008movement}. 

\subsubsection{Human Motion Analysis in Monocular Videos}
Human pose estimation aims to localize a human's joints in images or
videos. Human analysis in monocular videos often uses pose estimation as the initial step. State-of-the-art pose estimation systems are effective at localizing joints even when they are occluded
by objects or other parts of the body. We use a publicly available implementation of
a convolutional neural network-based pose estimator to track the wrist of the patient in our videos \citep{wei2016convolutional}.

Motion analysis in monocular videos often also relies on optical flow. Optical
flow measures the relative motion between the pixels in one frame and another.
Optical flow algorithms can be divided two categories: sparse and dense.
Sparse flow methods track only a sparse set of salient
points in the video, while dense flow methods 
measure motion at every pixel in the frame. We use sparse optical flow to
track background points for video stabilization \citep{lucas1981iterative}, and use dense optical flow
\citep{brox2009large} to refine the output of our pose estimator and to improve
the tracking of the patient's wrist in each video.

Our problem is similar to that of automatic human motion quality assessment.
\citet{pirsiavash2014assessing} use features based on the discrete cosine transform
(DCT) to estimate the judges' score for Olympic divers and figure skaters.
\citet{venkataraman2015dynamical} applied approximate entropy (ApEn) to the same task
and observed slight improvements.
\citet{venkataraman2013attractor} use shape-based dynamical features
to quantify levels of impairment of stroke survivors. These
methods are advantageous because they do not rely on domain-specific knowledge, but we found them to be insufficient for capturing the relevant motion characteristics in our videos. 


==> sections/3_dataset.tex <==
\section{The BARS Dataset}\label{sec:dataset}
We use a dataset of videos of ataxic patients to train a machine learning model that estimates the severity of motor impairment. Our dataset
consists of $90$ videos showing $43$ distinct subjects
performing several repetitions of the finger-to-nose test with one hand at a
time (\Cref{fig:vidPreview}). The videos were shot during clinic visits with handheld cameras.
All videos were labeled according to a version of the BARS that uses half-point
increments by the physician who created the scale. We treat these labels as
the gold standard on which we train our model. The scale ranges from $0$ (no impairment) to $4$ (so impaired as to be unable to complete the test), and the rating criteria includes motion characteristics such as instability of the finger or disjointed movements. \Cref{fig:fullHist} shows the
distribution of the severity ratings for the $90$ videos.
For several patients, there
are two videos for
each hand. The scores were
assigned separately for each hand, so a patient might have different ratings
for their right and left hands.

Some videos contain panning and zooming. We adjust for this by
using sparse optical flow to track points in the background, and then
estimating a similarity transformation from the tracked points to stabilize
each frame \citep{shi1994good,lucas1981iterative}. Because of the low number of
salient background points in some of the videos, only 61 videos were successfully
stabilized. We processed the remaining videos without stabilization.

% We didn't trim the video this time. We rely on cycle segmentation to detect
% the beginning and ending of action by looking at complete cycles

\begin{figure}[h]
    \begin{subfigure}[c]{.7\linewidth}
        %\centering
        \includegraphics[scale=0.4]{dataset.png}
        \caption{}
        \label{fig:vidPreview}
    \end{subfigure}%
    \begin{subfigure}[c]{.3\linewidth}
        %\centering
        \includegraphics[scale=0.22]{handHist.jpg}
        \caption{}
        \label{fig:fullHist}
    \end{subfigure}
    \caption{(a) A finger-to-nose exam. The patient alternates between touching
    his/her nose and the clinician's outstretched finger. Each video in our
    dataset contains at least two repetitions of this action. The eyes are
    occluded here for anonymity. (b) The
    distribution of severity ratings in the BARS dataset.}
\end{figure}




==> sections/4_featureextraction.tex <==
\section{Feature Extraction and Prediction Model}\label{sec:features}
We wish to extract features that
quantify relevant motion characteristics, including several characteristics described in the BARS guidelines. We extract these features from the motion signal of each patient's active hand. We use pose
estimation and optical flow to track the location of the patient's wrist and
head, segment the motion signal into cycles, and compute features from
the signal segments. This process is summarized in \Cref{fig:featextraction},
and explained in detail in the following subsections. 

\subsection{Head and Wrist Tracking}
\begin{figure}[h!]
	\centering
	\includegraphics[scale=0.15]{algo_diagram.png}
\caption{Our algorithm tracks the location of
the patient's active wrist, segments the location signal, computes
motion features, and then runs a linear regression to predict the BARS rating.}
\label{fig:featextraction}
\end{figure}
\subsubsection{Head and Wrist Location Estimates Using Pose Estimation}
We obtain the location of the
patient's active hand in each video frame. The quality of the videos, which are
representative of what might be captured in practice, make this a difficult
task. Most of the videos have low contrast, harsh lighting, and significant
motion blur, making local appearance-based tracking techniques such as sparse
point tracking \citep{lucas1981iterative} or mean-shift \citep{comaniciu2000real}
ineffective. In addition, there is significant variation in viewing angle
across videos, causing simple hand-recognition detectors to fail. We instead
rely on a more complex pose estimation system that calculates the likely
location of each body part in an image by leveraging information about the
configuration of the entire body. We start with a state-of-the-art pose estimation
system based on convolutional neural networks \citep{wei2016convolutional}. The system is designed to predict the location of several body joints in an image, such as the wrist
and the top of the neck (bottom of the head). We use the relative location of the wrist to the top 
of the neck to approximate the location of the patient's hand relative to
his/her head. Note that we do not estimate the location of the doctor's hand, as
it is not visible in some videos and cannot be reliably located in others due to low video quality. 

Using the pose estimator ``out of the box'' does not produce accurate wrist
location estimates. This is because the videos in our dataset contain
poses that are not well-represented in the dataset that the pose estimator was trained on, the MPII Human Pose dataset
\citep{andriluka20142d}. To
address this, we begin with the model trained on MPII, and further train or \textit{fine-tune} the network on a new annotated dataset of individuals
performing the finger-to-nose-test, none of whom appear in the BARS dataset. Our fine-tuning dataset
consists of $626$ images from $26$ distinct individuals; $507$ images are taken from videos of $15$ healthy individuals, and $119$ images are downloaded from
internet resources on ataxia. We annotated the locations of the joints in our dataset and fine-tuned the
network for $6,000$ iterations with a batch size of $8$. This small amount of additional training improved our wrist position estimates considerably; it reduced the Euclidean distance error by $31.9\%$ on a $70$-frame hand-annotated test set from the BARS videos.

\subsubsection{Temporal Regularization Using Optical Flow}
The pose estimator we use is designed for
images, and does not enforce temporal continuity between neighboring video
frames. We enforce this continuity by 
temporally smoothing the joint estimates for each frame, using
the estimates from neighboring frames and dense optical flow, as described in
\citet{charles2014upper}. We
further improve the smoothed wrist location estimates by constraining the
estimates to fall within the fastest-moving region, which we assume to contain the patient's active hand. We determine these regions
by computing dense trajectories from flow spanning multiple frames as described in
\citet{sundaram2010dense}, and then selecting the trajectories with the highest
amount of motion over the course of the video. 
This regularization further improves our tracking by $37.3\%$. Our final
average tracking error is $14.3\%$ of the range of patient's hand motion. An example of our
tracking results is shown in \Cref{fig:track}.

\begin{figure}
	\centering
	\includegraphics[scale=0.3]{track0.png}
	\includegraphics[scale=0.3]{track1.png}
	\includegraphics[scale=0.3]{track2.png}
        \caption{An example of our tracking results. The detected wrist position is marked in green, and the bottom of the head is marked in yellow.}
        \label{fig:track}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.6]{motionSigs_seg.jpg}
    \caption{Wrist $x$-position signals (relative to the head) for four different patients that were
    each given a severity rating of $2$. Notice that the signals differ considerably in
    shape and frequency. Segments are shown in alternating colors. Portions
    of the signal that did not fall within a full cycle (in gray) were
    discarded. }
    \label{fig:wristMotionSigs}
\end{figure}



\subsection{Cycle Segmentation}
\Cref{fig:wristMotionSigs} shows examples of the wrist $x$-position signal (relative to head) produced by our tracking algorithm.
The videos in our dataset contain varying numbers of repetitions of the finger-to-nose action.
To account for this, we assess the motion characteristics of each cycle independently. We first segment the wrist location signal in time. 
Our automated algorithm takes
as input the relative position of the patient's wrist to his/her head, and attempts
to segment cycles beginning when the wrist is halfway between the endpoints of the finger-to-nose action. We approximate the endpoints of the patient's hand motion using the minimum and maximum of the wrist position signal relative to the head. Since the beginning and the end
of the videos often include unrelated motions, we only compute the endpoint locations from the middle half of the signal.
For robustness against noise around the midpoints of the action, we use
hysteresis thresholding, a common thresholding technique used in signal processing, to detect the forward and backward portions of the
position signal. 
We define a
cycle to be finger-nose-finger or nose-finger-nose based on which designation
produces the higher number of cycles in a video, and exclude any portions of
the signal that do not fall within a complete cycle. The segments produced by 
our cycle segmentation algorithm are displayed in alternating colors in
\Cref{fig:wristMotionSigs}.


\subsection{Motion Features}
From these wrist location signal segments, we extract features that describe
characteristics of the patients' motion. To facilitate training on our relatively
small dataset, we designed these features based on the motion characteristics described in the BARS guidelines for rating the finger-to-nose test in
half-point increments. The total dimensionality is 14.

\subsubsection{Average Cycle Duration}
As described in the BARS guidelines, healthy patients are typically able to complete
each cycle of the finger-to-nose test more rapidly than impaired patients. We
compute the average time it takes for each patient to complete a cycle, as
well as just the nose-to-finger and finger-to-nose portions of the cycles. We
hypothesize that a difference in cycle length at low severities is more
discriminative than the same difference at high severities, and so we
use the logarithms of these values in our feature vector.

\subsubsection{Number of Direction Changes}
We capture the amount of oscillation in the patient's movements, an important rating criteria in the BARS, by counting the number of times the wrist
changes direction during the finger-to-nose action. We do this by counting the
number of sign changes in the first derivative of the wrist's $x-$ and $y-$position signals. Our features include the raw counts for both signals as well
as the counts normalized by the total number of cycles in the video. These
features also describe the patient's degree of dysmetria, since patients who
are more incoordinated have difficulty controlling the trajectory of their
hand during the test.

\subsubsection{Variation in Cycle Duration} 
Patients with more severe ataxia are unable to perform the
finger-to-nose action in a consistent manner. We capture this by computing the
standard deviations of the full cycle times, and the nose-to-finger and
finger-to-nose times.

\subsubsection{Approximate Entropy (ApEn)}
ApEn features describe the regularity of a signal by
segmenting signals into similar segments and computing the similarity of each
segment in higher dimensions
\citep{pincus1991approximate}. We followed \citet{venkataraman2015dynamical} and
computed ApEn features with similarity thresholds of $r=0.1,0.12,0.14,$ and $0.18$.
We found that an embedding dimension of $m=3$ performed best.

\subsection{Model}
Using the features described in the previous section, we train a linear
regression model to predict the BARS severity rating for each video. Though the
BARS rating is not necessarily a linear function of our feature space, we use
a simple model to avoid overfitting on our limited dataset. We use the LASSO technique,
a method for linear regression that includes a regularization term to help
with feature selection \citep{tibshirani1996regression}. We use
cross-validation to select the regularization parameter, and round the
predicted rating to the nearest valid BARS severity (which ranges from $0$ to $4$ in half-point increments).


==> sections/5_regression.tex <==
\section{Model}
Using the features described in the previous section, we train a linear
regression model to predict the BARS severity rating for each video. Though the
BARS rating is not necessarily a linear function of our feature space, we prefer to use
a simpler model to avoid overfitting on our limited dataset. We use the LASSO technique,
a method for linear regression that includes a regularization term to help
with feature selection \citep{tibshirani1996regression}. We use
cross-validation to select the regularization parameter, and round the
predicted rating to the nearest valid BARS severity rating (which goes in half
point increments from 0 to 4).

%We split our BARS dataset into training and
%holdout sets such that training set contained at least one video of each
%severity rating. Since there are multiple videos of each subject, the subjects
%were split such that each subject appeared in either the training set or in
%the holdout set but not both. This resulted in $28$ training subjects and $12$
%test subjects, with the severities distributed similarly (Figures
%\ref{fig:trainHist} and \ref{fig:testHist}). Unfortunately, we had only one
%subject each at severity levels 3.5 and 4. We included these subjects in the
%training set.

%\begin{figure}
%\centering
%    \subfigure[Full dataset ($84$ videos, $40$ subjects).] {
%        \centering
%        \includegraphics[scale=0.5]{handHist.png}
%    } \label{fig:fullHist}
%~
%    \subfigure[Training set ($60$ videos, $28$ subjects).] {
%        \centering
%        \includegraphics[scale=0.5]{trainHist.png}
%    } \label{fig:trainHist}
%~
%   \subfigure[Test set ($24$ videos, $12$ subjects).] {
%        \centering
%        \includegraphics[scale=0.5]{testHist.png}
%    } \label{fig:testHist}
%\caption{Distribution of BARS severity ratings for our videos. }
%\end{figure}


%While this is not ideal, each of the error we report was a result of
%predicting severity rating with a regressor that has not seen that data point
%before.

%Feature selection is still an open problem in machine-learning community. We
%used heuristic to narrow down the list of feature. Each feature individually
%were used to rank the data, and we chose ten features that rank our data most
%closely to expert ratings. Next section discuss the result of our prediction.


==> sections/6_results.tex <==
\section{Evaluation} \label{sec:learning-result}
Because of the limited number of examples in our dataset, we use leave-one-patient-out cross
validation to test our models. This approach allows us to train each model
with the maximum amount of data, and evaluate the model's performance on a
patient that it has not yet seen. 

%\begin{figure}[h]
    %\centering
    %\includegraphics[scale=0.35]{errorDist_all.png}
    %\caption{Distribution of absolute errors in our leave-one-patient-out evaluation.}
    %\label{fig:errordist}
%\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{pred_v_gt.png}
    \caption{Our system's predictions versus the gold standard ratings on the
    full $90$ video dataset. Dot area and the associated number represent the number of videos. Perfect
    prediction is represented by the red line. Our mean
    absolute error was $0.333$ and our correlation with the gold standard labels
    was $0.856$. This is comparable to the performance of skilled clinicians.
    }
    \label{fig:predvgt}
\end{figure}

\subsection{Prediction Error}
Our model performs reasonably well in learning the gold standard ratings. \Cref{fig:predvgt} shows our predictions versus the ground truth severity
ratings. 
Most (87.8\%) of our models' prediction errors are less than one level on
the BARS. Only one video produced an absolute error greater than 1 point. In this
case, tracking noise caused a cycle segmentation error that combined two cycles into one.

\subsection{Comparison with Physicians Specializing in Ataxia}
\label{sec:humperf}
We have shown that our system can learn the gold standard labels with low error, but is it good enough for clinical use? We demonstrate that our system performs comparably with the current clinical state-of-the-art: human raters using a
rating scale such as the BARS. We collected
ratings for $32$ test videos from 6 ataxia specialists, all of whom are
practicing physicians as well as members of the Clinical Research Consortium for
Spinocerebellar Ataxias. All of the specialists had used ataxia rating scales such as the SARA before, but none had prior experience with the
half-point BARS. They were provided with textual descriptions of each BARS
severity and were all shown the same $1-3$ example videos for each severity
level. Each specialist rated each video independently and in randomized order.
The test videos were hand-selected so that they had as uniform a severity distribution, and as
few common patients with the example set as possible. No videos appeared in both
the example set and the test set; however, some videos from the same patient taken during different clinical visits appear in both. While the ataxia specialist raters did not learn from as many videos as our
system did, they have the advantage of learning from textual descriptions in
the BARS, as well as their prior expertise in treating ataxia. This arrangement is
representative of how human raters would be trained
in practice.


\begin{figure}[h]
	\centering
	\includegraphics[scale=0.3]{doc_v_us_err.png}
~
	\includegraphics[scale=0.3]{doc_v_us_corr.png}
        \caption{Comparison of our system's performance to each of the ataxia specialist
            raters with respect to the gold standard label. The error bars represent
            the standard error of the mean.
        }
        \label{fig:summary_metric}
\end{figure}

We first compare the performance of our system and the ataxia specialists on learning the gold standard labels. \Cref{fig:summary_metric} shows that our predictions fall within the range of the specialists in terms of mean absolute error and correlation with the gold
standard. On average, our system achieves an absolute error of $0.344$ and a
correlation of $0.868$ whereas the specialists achieve $0.378$ mean
absolute error, and $0.872$ correlation. This indicates that our system can learn the BARS as well as expert
physicians.
%can produce predictions that are consistent with the provided labels, an important characteristic for an objective rating system.

%The mean absolute error of our system and the average of the specialists were $0.344$ and $0.378$ respectively, and the correlations were $0.868$ and $0.872$ respectively.

\begin{figure}[h]
        \centering
        \includegraphics[scale=0.5]{doctorratings_sortedbymean.jpg}
            \caption{
                Range of ataxia specialists' ratings for each test videos.
                Our rating (red) was almost always within the range of the ataxia
                specialists' ratings (yellow). 
            }
    \label{fig:docrange}
\end{figure}

Additionally, we compare our predictions with inter-rater variability among the
specialists. \Cref{fig:docrange} compares our prediction with the specialists'
ratings for individual videos.
In this result, we make no distinction between the gold standard rater and the
other specialists, to more accurately capture inter-rater variability among
ataxia specialists.
Our predictions were consistently within the range
of inter-rater variability. Our prediction falls within the range of specialist
ratings 78\% of the time, and within $0.5$ points of the range for all but one
video, where a low severity patient moved their finger slowly, causing us to
overestimate their severity rating by 1.
%Because the gold standard
%ratings are also given by a specialist, they contribute to inter-rater
%variability, so we consider them as one of the
%specialist ratings.

%That video was of a patient of severity rating
%of 0.5 who performed the maneuver slowly, causing our algorithm to predict
%rating 1 point above the ratings given by specialists. This highlights a
%limitation of our algorithm, which we discuss in greater detail in
%\Cref{sec:limitation}.


Our results indicate that our system performs comparably to neurologists specializing in ataxia. In areas where
    ataxia specialists are not available, our system may provide a more accurate evaluation of ataxia than human clinicians. Our system could also be useful for producing more
    consistent ratings of ataxia between different clinical visits, or between different clinicians.
    



==> sections/7_discussion.tex <==
\section{Discussion and Conclusion}
\label{sec:limitation}
We described an automatic, video-based system for quantifying the severity of motion impairment of ataxic
patients performing the finger-to-nose test described in the Brief Ataxia
Rating Scale (BARS). The system is designed with consideration for the low video quality that one might expect from clinical settings; it is robust to variations in camera angle, harsh lighting conditions and motion blur. Our system uses convolutional neural network-based pose
estimation and optical flow to track the location of a patient's wrist and
head. From the wrist motion signals, we extract
features such as average cycle time and amount of oscillation. We use these features to build
a linear regression model to predict the severity rating of the patient's
action. We show that our system can predict BARS ratings with comparable accuracy to experienced ataxia specialists. More importantly, most of our system's predictions fall within the range of ratings supplied by these specialists. This suggests that our system might be a suitable
observer-independent alternative to traditional human-administered rating
scales. 
%Our predictions are, on average, slightly more accurate than those of  

%Our system could benefit from more training data in several ways.
%Firstly, 
Our system is limited to using a simple linear model that may not capture all of the relevant
characteristics of the motion. It tends to
overestimate the rating for lower severity videos, and underestimate the rating on higher
severity videos. A larger training set would permit the use of a more complex
model than linear regression, which might help capture these more complicated cases. 

We hope that this work will lead to a system that can be used in the management of movement disorders in clinical
or home settings, and to reduce observer bias in clinical trials. The automatic and consistent ratings provided by such a system can improve the monitoring and treatment of these disorders. Such a system
would be particularly beneficial in many parts of the country that do not have
access to specialists.

 \break
%neurologists or physicians with little experience in ataxia.





%Our dataset contains a limited number of examples for the higher severities -- the videos with severity ratings of $3.5$ and $4$ were all of
%the same patient. While our system performed reasonably well on these videos,
%it is unclear if our
%system will generalize well for other severely impaired patients.
%Our model could be made more generalizable by obtaining
%more videos of severely impaired patients, making the dataset more evenly
%distributed over the range of the BARS severity ratings. 


==> sections/8_conclusion.tex <==
\section{Conclusion}
We describe an automatic, video-based method for quantifying the severity of motion
impairment, and use the method to predict the severity rating of ataxic
patients performing the finger-to-nose test described in the Brief Ataxia
Rating Scale (BARS). Our method uses convolutional neural network-based pose
estimation and optical flow to track the location of a patient's wrist and
head. This tracking method 
is robust to the variations in camera angle and lighting conditions present in our dataset. We
segment the resulting wrist position signal into cycles, and extract
features such as average cycle time and amount of oscillation from these
signal segments based on the BARS guidelines. We use these features to build
a linear regression model to predict the severity rating of the patient's
action. 

We demonstrate that our model performs comparably to ataxia specialists. Our
predictions fall consistently within the range of inter-rater variability.  
This shows that our system might be a suitable
observer-independent alternative to traditional human-administered rating
scales. Such a system could be used to improve the management of the disease in clinical
or home settings, or to reduce observer bias in clinical trials. This system
would be particularly beneficial in many parts of the country that do not have
access to ataxia specialists, since it may be able to provide more consistent
ratings than neurologists or physicians with little experience in ataxia.
We believe that our system is an important step towards the automatic evaluation
of movement disorders in real clinical environments.


